Universal Network Representation for Heterogeneous Information Networks

Network representation aims to represent the nodes in a network as continuous and compact vectors, and has attracted much attention in recent years due to its ability to capture complex structure relationships inside networks. However, existing network representation methods are commonly designed for homogeneous information networks where all the nodes (entities) of a network are of the same type, e.g., papers in a citation network. In this paper, we propose a universal network representation approach (UNRA), that represents different types of nodes in heterogeneous information networks in a continuous and common vector space. The UNRA is built on our latest mutually updated neural language module, which simultaneously captures inter-relationship among homogeneous nodes and node-content correlation. Relationships between different types of nodes are also assembled and learned in a unified framework. Experiments validate that the UNRA achieves outstanding performance, compared to six other state-of-the-art algorithms, in node representation, node classification, and network visualization. In node classification, the UNRA achieves a 3\% to 132\% performance improvement in terms of accuracy.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Universal representation in hetergenious neural network/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Universal representation in hetergenious neural network/algorithm_comparison.tex <==
\begin{table*}[htbp]
	\caption{Algorithms for clustering network data with node content information.}
    \label{tab:algorithm_comparison}%
    \centering
    \begin{tabular}{cccccc}
    \toprule
         %& Auxiliary data    & Auxiliary data   \\
        Algorithms & Network Structure? & Node Features? &Overlapping Node Clustering? & Feature Clustering? &Group Function (Intepretation) \\
          \midrule
          K-means& $\times$ & $\surd$&$\times$&$\times$&$\times$\\
                     
          \midrule          
         GNMF \cite{cai2008non}& $\surd$ & $\surd$&$\times$&$\surd$&$\surd$\\

        DRCC \cite{gu2009co} & $\surd$ & $\surd$&$\times$&$\surd$&$\surd$\\
        FNMTF \cite{wang2011fast} & $\surd$ & $\surd$&$\times$&$\surd$&$\surd$\\   
          \midrule
      
          BigClam \cite{yang2013overlapping}& $\surd$ & $\times$&$\surd$&$\times$&$\times$\\
          AGMFit \cite{yang2012community} & $\surd$ & $\times$&$\surd$&$\times$&$\times$\\
          
          \midrule
          Censa \cite{yang2013community} & $\surd$ & $\surd$&$\surd$&$\times$&$\surd$\\				
		Circle \cite{leskovec2012learning} & $\surd$ & $\surd$&$\surd$&$\times$&$\surd$\\
        Ours & $\surd$ & $\surd$&$\surd$&$\surd$&$\surd$\\

    \bottomrule
    \end{tabular}%
\end{table*}


==> Universal representation in hetergenious neural network/casestudy.tex <==
\begin{table}
  \centering
  \caption{outputs from representations. The matched is marked with \astrosun}
    \begin{tabular}{@{}*{2}{p{.47\textwidth}@{}}}
    \toprule
    \textbf{Input}: Learning in Neural Networks \\
    \midrule
    URHN:  \\
    1. Adjoint-Functions and Temporal Learning Algorithms in Neural Networks \astrosun\\
    2. Bit-Serial Neural Networks \astrosun \\
    3. An Information-theoretic Learning Algorithm for Neural Network Classification \astrosun \\
    4. Polynomial Time Algorithms for Learning Neural Nets \astrosun \\
    5. Training of Large-Scale Feed-Forward Neural Networks \astrosun \\
    \midrule
   Doc2Vec: \\
    1. Non-Cumulative Learning in METAXA.3 \\
    2. Learning Filaments \\
    3. Learning of Kernel Functions in Support Vector Machines \\
    4. Incremental Learning in SwiftFile \\
    5. Learning While Searching in Constraint-Satisfaction-Problems \\
    \midrule
    DeepWalk:\\
    1. Estimating image motion from smear: a sensor system and extensions \\
    2. Inferring 3D Volumetric Shape of Both Moving Objects and Static Background Observed by a Moving Camera\\
    3. Secure face biometric verification in the randomized Radon space\\
    4. An Ensemble Prior of Image Structure for Cross-Modal Inference\\
    5. Closed Non-derivable Itemsets\\
    \bottomrule
    \end{tabular}%
  \label{tab:casestudy}%
\end{table}%

==> Universal representation in hetergenious neural network/datasets.tex <==
\begin{table*}[htpb]
\small
  \centering
  \caption{Enterprise Social Network Datasets Used in the Paper}
    \begin{tabular}{lcccccl}
    \toprule
    Data Set & \#Paper\_Nodes & \#Author\_Nodes & \#Paper\_Edges & \#Author\_Edges & \#Content\_words  & \#Labela \\
    \midrule
    DBLP & 56,503 & 58,279   & 106,752 & 142,581  & 3,262,885 & 4     \\
    CiteSeerX-Avs   &  18,720 & 40,139   & 54,601 & 41,458  & 2,649,720  & 5    \\
    CiteSeerX-M10 & 10,310 & 21,289   & 77,218 & 21,966  & 1,516,893 & 10     \\
    \bottomrule
    \end{tabular}%
  \label{tab:datasets}%
\end{table*}%

==> Universal representation in hetergenious neural network/f1k11.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=11}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 11 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0.338 & 0.132 & 0.281 & 0.294 & 0.318 & 0.168 & 0.198 & 0.164 & 0.271 & \textbf{0.393}\\
    NBA   & \textbf{0.950} & 0.461 & 0.709 & 0.698 & 0.633 & 0.393 & 0.433 & 0.565 & 0.418 & 0.5368\\
    TwitterAU & \textbf{0.808} & 0.539 & 0.406 & 0.601 & 0.359 & 0.363 & 0.275 & 0.440 & 0.278 & 0.443\\
    SonyPictures & 0.439 & 0.210 & 0.240 & 0.119 & 0.233 & 0.332 & 0.420 & 0.394 & 0.430 & \textbf{0.487}\\
    AustralianLabor & \textbf{0.860} & 0.395 & 0.458 & 0.396 & 0.478 & 0.306 & 0.408 & 0.346 & 0.494 & 0.767\\
    WhiteHouse & \textbf{0.863} & 0.149 & 0.310 & 0.430 & 0.295 & 0.291 & 0.313 & 0.297 & 0.502 & 0.652\\
    MercedesBenz & \textbf{0.787} & 0.103 & 0.520 & 0.367 & 0.405 & 0.233 & 0.271 & 0.318 & 0.383 & 0.383\\
    Techreview & 0.442 & 0.201 & 0.267 & 0.221 & 0.255 & 0.247 & 0.176 & 0.248 & 0.342 & \textbf{0.463}\\
    Cambridge\_Uni & \textbf{0.652} & 0.167 & 0.527 & 0.316 & 0.527 & 0.174 & 0.087 & 0.256 & 0.261 & 0.329\\
    The\_Nationals & \textbf{0.850} & 0.403 & 0.619 & 0.661 & 0.403 & 0.624 & 0.624 & 0.558 & 0.697 & 0.407\\
    Greens & 0.413 & 0.249 & 0.389 & 0.335 & 0.358 & 0.222 & 0.169 & 0.246 & 0.341 & \textbf{0.714}\\
    MGM\_Studios & \textbf{0.704} & 0.257 & 0.515 & 0.298 & 0.427 & 0.318 & 0.463 & 0.463 & 0.413 & 0.612\\
    BBCNews & 0.554 & 0.205 & 0.658 & 0.495 & \textbf{0.712} & 0.223 & 0.079 & 0.280 & 0.363 & 0.381\\
    \textbf{Average} & \textbf{0.666} & 0.267 & 0.454 & 0.402 & 0.416 & 0.299 & 0.301 & 0.352 & 0.399 & 0.505\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k11}%
\end{table*}%

==> Universal representation in hetergenious neural network/f1k5.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=5}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 5 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0. 432 & 0.215 & 0.181 & 0.075 & 0.177 & 0.294 & 0.216 & 0.222 & 0.460 & \textbf{0.686}\\
    NBA   & \textbf{0.922} & 0.641 & 0.698 & 0.633 & 0.728 & 0.467 & 0.393 & 0.610 & 0.458 & 0.368\\
    TwitterAU & \textbf{0.834} & 0.444 & 0.203 & 0.133 & 0.207 & 0.440 & 0.280 & 0.687 & 0.484 & 0.833\\
    SonyPictures & \textbf{0.527} & 0.420 & 0.330 & 0.113 & 0.337 & 0.338 & 0.192 & 0.501 & 0.348 & 0.224\\
    AustralianLabor & \textbf{0.783} & 0.366 & 0.457 & 0.603 & 0.442 & 0.302 & 0.341 & 0.397 & 0.632 &  0.157\\
    WhiteHouse & \textbf{0.924} & 0.297 & 0.285 & 0.459 & 0.279 & 0.311 & 0.217 & 0.265 & 0.504 & 0.248\\
    MercedesBenz & \textbf{0.757} & 0.238 & 0.516 & 0.420 & 0.486 & 0.291 & 0.363 & 0.360 & 0.482 & 0.383\\
    Techreview & 0.462 & 0.224 & \textbf{0.757} & 0.176 & 0.746 & 0.248 & 0.242 & 0.218 & 0.367 & 0.522\\
    Cambridge\_Uni & \textbf{0.713} & 0.229 & 0.295 & 0.197 & 0.289 & 0.244 & 0.155 & 0.237 & 0.366 & 0.633\\
    The\_Nationals & \textbf{0.962} & 0.356 & 0.737 & 0.622 & 0.716 & 0.663 & 0.658 & 0.528 & 0.676 & 0.593\\
    Greens & 0.379 & 0.346 & 0.510 & 0.447 & 0.523 & 0.318 & 0.319 & 0.340 & 0.517 & \textbf{0.597}\\
    MGM\_Studios & \textbf{0.776} & 0.458 & 0.515 & 0.552 & 0.583 & 0.297 & 0.189 & 0.578 & 0.462 & 0.522\\
    BBCNews & \textbf{0.748} & 0.291 & 0.577 & 0.252 & 0.559 & 0.303 & 0.160 & 0.285 & 0.510 & 0.605\\
    \textbf{Average} & \textbf{0.681} & 0.348 & 0.466 & 0.396 & 0.467 & 0.347 & 0.286 & 0.402 & 0.482 & 0.490\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k5}%
\end{table*}%

==> Universal representation in hetergenious neural network/f1k7.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=7}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 7 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0.393 & 0.182 & 0.424 & 0.086 & 0.363 & 0.236 & 0.162 & 0.179 & 0.391 & \textbf{0.800}\\
    NBA   & 0.788 & 0.410 & 0.786 & 0.769 & \textbf{0.791} & 0.403 & 0.374 & 0.575 & 0.428 & 0.324\\
    TwitterAU & \textbf{0.858} & 0.463 & 0.242 & 0.309 & 0.254 & 0.507 & 0.206 & 0.654 & 0.377 &  0.724\\
    SonyPictures & \textbf{0. 496} & 0.171 & 0.291 & 0.093 & 0.330 & 0.399 & 0.452 & 0.492 & 0.410 & 0.237\\
    AustralianLabor & \textbf{0.897} & 0.442 & 0.503 & 0.452 & 0.614 & 0.386 & 0.466 & 0.404 & 0.601 & 0.677\\
    WhiteHouse & \textbf{0.779} & 0.253 & 0.465 & 0.520 & 0.391 & 0.318 & 0.210 & 0.361 & 0.486 & 0.460\\
    MercedesBenz & \textbf{0.568} & 0.087 & 0.538 & 0.500 & 0.451 & 0.232 & 0.273 & 0.283 & 0.390 & 0.281\\
    Techreview & 0.302 & 0.183 & \textbf{0.410} & 0.320 & 0.380 & 0.211 & 0.174 & 0.216 & 0.314 & 0.209\\
    Cambridge\_Uni & \textbf{0.701} & 0.169 & 0.463 & 0.236 & 0.478 & 0.241 & 0.114 & 0.226 & 0.356 & 0.592\\
    The\_Nationals & \textbf{0.869} & 0.370 & 0.656 & 0.636 & 0.642 & 0.618 & 0.651 & 0.623 & 0.679 & 0.593 \\
    Greens & 0.440 & 0.240 & 0.415 & 0.488 & 0.458 & 0.230 & 0.226 & 0.241 & 0.407 & \textbf{0.636}\\
    MGM\_Studios & \textbf{0.704} & 0.354 & 0.456 & 0.365 & 0.569 & 0.325 & 0.359 & 0.546 & 0.416 & 0.493\\
    BBCNews & \textbf{0.634} & 0.261 & 0.630 & 0.373 & 0.605 & 0.254 & 0.116 & 0.314 & 0.475 & 0.375\\
    \textbf{Average} & \textbf{0.643} & 0.276 & 0.483 & 0.396 & 0.487 & 0.335 & 0.291 & 0.394 & 0.441 & 0.492\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k7}%
\end{table*}%

==> Universal representation in hetergenious neural network/f1k9.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=9}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 9 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0.366 & 0.192 & 0.257 & 0.226 & 0.272 & 0.174 & 0.231 & 0.159 & 0.319 & \textbf{0.729}\\
    NBA   & \textbf{0.941} & 0.437 & 0.709 & 0.652 & 0.689 & 0.419 & 0.399 & 0.501 & 0.432 & 0.493\\
    TwitterAU & \textbf{0.625} & 0.434 & 0.455 & 0.350 & 0.453 & 0.415 & 0.285 & 0.529 & 0.329 & 0.540\\
    SonyPictures & 0.451 & 0.172 & 0.240 & 0.116 & 0.224 & 0.308 & 0.441 & 0.414 & 0.426 & \textbf{0.513}\\
    AustralianLabor & \textbf{0.798} & 0.405 & 0.433 & 0.378 & 0.490 & 0.325 & 0.462 & 0.445 & 0.574 & 0.689\\
    WhiteHouse & \textbf{0.825} & 0.122 & 0.357 & 0.356 & 0.320 & 0.297 & 0.207 & 0.321 & 0.494 & 0.665\\
    MercedesBenz & \textbf{0.714} & 0.115 & 0.521 & 0.410 & 0.430 & 0.249 & 0.263 & 0.375 & 0.396 & 0.359\\
    Techreview & 0.384 & 0.161 & 0.348 & 0.321 & 0.303 & 0.261 & 0.193 & 0.253 & 0.371 & \textbf{0.418}\\
    Cambridge\_Uni & \textbf{0.810} & 0.187 & 0.684 & 0.261 & 0.741 & 0.205 & 0.097 & 0.274 & 0.315 & 0.469\\
    The\_Nationals & 0.549 & 0.385 & 0.586 & 0.468 & 0.404 & 0.624 & 0.566 & 0.578 & \textbf{0.734} & 0.593\\
    Greens & 0.375 & 0.165 & 0.295 & 0.379 & 0.414 & 0.256 & 0.177 & 0.211 & 0.351 & \textbf{0.669}\\
    MGM\_Studios & \textbf{0.723} & 0.275 & 0.239 & 0.258 & 0.534 & 0.270 & 0.473 & 0.671 & 0.389 & 0.478\\
    BBCNews & 0.678 & 0.244 & \textbf{0.760} & 0.459 & 0.732 & 0.237 & 0.093 & 0.279 & 0.406 & 0.426\\
    \textbf{Average} & \textbf{0.634} & 0.254 & 0.453 & 0.402 & 0.462 & 0.311 & 0.299 & 0.385 & 0.426 & 0.542\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k9}%
\end{table*}%

==> Universal representation in hetergenious neural network/macro_f1_Avs.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Macro F1 Avs}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & LDA & TADW  & RTM \\
    \midrule
    10\% & 0.76084 & 0.75957 & \textbf{0.764392} & 0.369541 & 0.764391 & 0 & 0 & 0 & 0 \\
    20\%   & \textbf{0.810043} & 0.807608 & 0.781474 & 0.366090 & 0.798168 & 0 & 0 & 0 & 0 \\
    30\% & \textbf{0.851001} & 0.837247 & 0.782137 & 0.363368 & 0.809289 & 0 & 0 & 0 & 0 \\
    40\% & \textbf{0.866406} & 0.863792 & 0.785615 & 0.362034 & 0.810925 & 0 & 0 & 0 & 0 \\
    50\% & \textbf{0.877181} & 0.868892 & 0.788058 & 0.363419 & 0.820524 & 0 & 0 & 0 & 0 \\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%

==> Universal representation in hetergenious neural network/macro_f1_M10.tex <==
%\newcolumntype{c}{>{\columncolor{LightCyan}}r}
\begin{table*}[htbp]
  \centering
  \caption{Macro F1 M10}
    \begin{tabular}{lcrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & TADW\\
    \midrule
  %  \rowcolor{LightCyan}
    10\% & \textbf{0.779} & 0.75957 & 0.684668 & 0.333647 & 0.689372 & 0.53234 & 0.7298\\
    20\% & \textbf{0.830} & 0.807608 & 0.729520 & 0.368398 & 0.736581 & 0.561233 & 0.7480 \\
    30\% & \textbf{0.851001} & 0.837247 & 0.756816 & 0.374327 & 0.770119 & 0.568377 & 0.7536 \\
    40\% & \textbf{0.866406} & 0.863792 & 0.768484 & 0.377251 & 0.788898 & 0.575826 & 0.7545 \\
    50\% & \textbf{0.877181} & 0.868892 & 0.762745 & 0.377689 & 0.786972 & 0.582193 & 0.7543\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%

==> Universal representation in hetergenious neural network/macro_f1_dblp.tex <==
%\newcolumntype{c}{>{\columncolor{LightCyan}}r}
\begin{table*}[htbp]
  \centering
  \caption{Macro F1 DBLP}
    \begin{tabular}{lcrrrrrrrr}
    \toprule
    Training size & UNRA  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & TADW\\
    \midrule
  %  \rowcolor{LightCyan}
    10\% & \textbf{0.732} & 0.715 & 0.638 & 0.385 & 0.659 & 0.431 & 0.670\\
    20\% & \textbf{0.732} & 0.727 & 0.644 & 0.320 & 0.669 & 0.439 & 0.698 \\
    30\% & \textbf{0.736} & 0.730 & 0.643 & 0.317 & 0.668 & 0.445 & 0.709 \\
    40\% & \textbf{0.739} & 0.736 & 0.643 & 0.308 & 0.668 & 0.446 & 0.711 \\
    50\% & \textbf{0.742} & 0.738 & 0.650 & 0.320 & 0.675 & 0.446 & 0.712\\
    \bottomrule
    \end{tabular}%
  \label{tab:dblpmacro}%
\end{table*}%

==> Universal representation in hetergenious neural network/micro_f1_Avs.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Micro F1 Avs}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & LDA & TADW  & RTM \\
    \midrule
    10\% & \textbf{0.791896} & 0.791034 & 0.788818 & 0.498516 & 0.791785 & 0 & 0 & 0 & 0 \\
    20\%   & \textbf{0.841052} & 0.836081 & 0.804554 & 0.498464 & 0.822449 & 0 & 0 & 0 & 0 \\
    30\% & \textbf{0.870722} & 0.861577 &  0.805861 & 0.500305 & 0.833639 & 0 & 0 & 0 & 0 \\
    40\% & \textbf{0.885548} & 0.87989 & 0.808137 & 0.497418 & 0.833957 & 0 & 0 & 0 & 0 \\
    50\% & \textbf{0.892726} & 0.885936 & 0.809081 & 0.500214 & 0.840919 & 0 & 0 & 0 & 0 \\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%

==> Universal representation in hetergenious neural network/micro_f1_M10.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Micro F1 M10}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & TADW \\
    \midrule
    10\% & \textbf{0.806660} & 0.791034 & 0.717642 & 0.418472 & 0.710098 & 0.604661 & 0.7309 \\
    20\%   & \textbf{0.848206} & 0.836081 & 0.763337 & 0.467022 & 0.761882 & 0.628977 & 0.7482 \\
    30\% & \textbf{0.870722} & 0.861577 &  0.786199 & 0.476375 & 0.795067 & 0.641788 & 0.7490 \\
    40\% & \textbf{0.885548} & 0.87989 & 0.795668 & 0.483834 & 0.812803 & 0.651029 & 0.7591 \\
    50\% & \textbf{0.892726} & 0.885936 & 0.789331 & 0.485936 & 0.810475 & 0.655983 & 0.7606 \\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%

==> Universal representation in hetergenious neural network/micro_f1_dblp.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Micro F1 DBLP}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    Training size & UNRA  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & TADW \\
    \midrule
    10\% & \textbf{0.791} & 0.777 & 0.717 & 0.455 & 0.728 & 0.488 & 0.662 \\
    20\%   & \textbf{0.792} & 0.787 & 0.722 & 0.478 & 0.737 & 0.494 & 0.670\\
    30\% & \textbf{0.795} & 0.788 &  0.722 & 0.478 & 0.736 & 0.498 & 0.711 \\
    40\% & \textbf{0.797} & 0.793 & 0.722 & 0.479 & 0.739 & 0.499 & 0.705 \\
    50\% & \textbf{0.798} & 0.798 & 0.724 & 0.482 & 0.740 & 0.511 & 0.716 \\
    \bottomrule
    \end{tabular}%
  \label{tab:dblpmicro}%
\end{table*}%

==> algorithm_comparison.tex <==
\begin{table*}[htbp]
	\caption{Algorithms for clustering network data with node content information.}
    \label{tab:algorithm_comparison}%
    \centering
    \begin{tabular}{cccccc}
    \toprule
         %& Auxiliary data    & Auxiliary data   \\
        Algorithms & Network Structure? & Node Features? &Overlapping Node Clustering? & Feature Clustering? &Group Function (Intepretation) \\
          \midrule
          K-means& $\times$ & $\surd$&$\times$&$\times$&$\times$\\
                     
          \midrule          
         GNMF \cite{cai2008non}& $\surd$ & $\surd$&$\times$&$\surd$&$\surd$\\

        DRCC \cite{gu2009co} & $\surd$ & $\surd$&$\times$&$\surd$&$\surd$\\
        FNMTF \cite{wang2011fast} & $\surd$ & $\surd$&$\times$&$\surd$&$\surd$\\   
          \midrule
      
          BigClam \cite{yang2013overlapping}& $\surd$ & $\times$&$\surd$&$\times$&$\times$\\
          AGMFit \cite{yang2012community} & $\surd$ & $\times$&$\surd$&$\times$&$\times$\\
          
          \midrule
          Censa \cite{yang2013community} & $\surd$ & $\surd$&$\surd$&$\times$&$\surd$\\				
		Circle \cite{leskovec2012learning} & $\surd$ & $\surd$&$\surd$&$\times$&$\surd$\\
        Ours & $\surd$ & $\surd$&$\surd$&$\surd$&$\surd$\\

    \bottomrule
    \end{tabular}%
\end{table*}


==> f1k11.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=11}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 11 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0.338 & 0.132 & 0.281 & 0.294 & 0.318 & 0.168 & 0.198 & 0.164 & 0.271 & \textbf{0.393}\\
    NBA   & \textbf{0.950} & 0.461 & 0.709 & 0.698 & 0.633 & 0.393 & 0.433 & 0.565 & 0.418 & 0.5368\\
    TwitterAU & \textbf{0.808} & 0.539 & 0.406 & 0.601 & 0.359 & 0.363 & 0.275 & 0.440 & 0.278 & 0.443\\
    SonyPictures & 0.439 & 0.210 & 0.240 & 0.119 & 0.233 & 0.332 & 0.420 & 0.394 & 0.430 & \textbf{0.487}\\
    AustralianLabor & \textbf{0.860} & 0.395 & 0.458 & 0.396 & 0.478 & 0.306 & 0.408 & 0.346 & 0.494 & 0.767\\
    WhiteHouse & \textbf{0.863} & 0.149 & 0.310 & 0.430 & 0.295 & 0.291 & 0.313 & 0.297 & 0.502 & 0.652\\
    MercedesBenz & \textbf{0.787} & 0.103 & 0.520 & 0.367 & 0.405 & 0.233 & 0.271 & 0.318 & 0.383 & 0.383\\
    Techreview & 0.442 & 0.201 & 0.267 & 0.221 & 0.255 & 0.247 & 0.176 & 0.248 & 0.342 & \textbf{0.463}\\
    Cambridge\_Uni & \textbf{0.652} & 0.167 & 0.527 & 0.316 & 0.527 & 0.174 & 0.087 & 0.256 & 0.261 & 0.329\\
    The\_Nationals & \textbf{0.850} & 0.403 & 0.619 & 0.661 & 0.403 & 0.624 & 0.624 & 0.558 & 0.697 & 0.407\\
    Greens & 0.413 & 0.249 & 0.389 & 0.335 & 0.358 & 0.222 & 0.169 & 0.246 & 0.341 & \textbf{0.714}\\
    MGM\_Studios & \textbf{0.704} & 0.257 & 0.515 & 0.298 & 0.427 & 0.318 & 0.463 & 0.463 & 0.413 & 0.612\\
    BBCNews & 0.554 & 0.205 & 0.658 & 0.495 & \textbf{0.712} & 0.223 & 0.079 & 0.280 & 0.363 & 0.381\\
    \textbf{Average} & \textbf{0.666} & 0.267 & 0.454 & 0.402 & 0.416 & 0.299 & 0.301 & 0.352 & 0.399 & 0.505\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k11}%
\end{table*}%

==> f1k5.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=5}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 5 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0. 432 & 0.215 & 0.181 & 0.075 & 0.177 & 0.294 & 0.216 & 0.222 & 0.460 & \textbf{0.686}\\
    NBA   & \textbf{0.922} & 0.641 & 0.698 & 0.633 & 0.728 & 0.467 & 0.393 & 0.610 & 0.458 & 0.368\\
    TwitterAU & \textbf{0.834} & 0.444 & 0.203 & 0.133 & 0.207 & 0.440 & 0.280 & 0.687 & 0.484 & 0.833\\
    SonyPictures & \textbf{0.527} & 0.420 & 0.330 & 0.113 & 0.337 & 0.338 & 0.192 & 0.501 & 0.348 & 0.224\\
    AustralianLabor & \textbf{0.783} & 0.366 & 0.457 & 0.603 & 0.442 & 0.302 & 0.341 & 0.397 & 0.632 &  0.157\\
    WhiteHouse & \textbf{0.924} & 0.297 & 0.285 & 0.459 & 0.279 & 0.311 & 0.217 & 0.265 & 0.504 & 0.248\\
    MercedesBenz & \textbf{0.757} & 0.238 & 0.516 & 0.420 & 0.486 & 0.291 & 0.363 & 0.360 & 0.482 & 0.383\\
    Techreview & 0.462 & 0.224 & \textbf{0.757} & 0.176 & 0.746 & 0.248 & 0.242 & 0.218 & 0.367 & 0.522\\
    Cambridge\_Uni & \textbf{0.713} & 0.229 & 0.295 & 0.197 & 0.289 & 0.244 & 0.155 & 0.237 & 0.366 & 0.633\\
    The\_Nationals & \textbf{0.962} & 0.356 & 0.737 & 0.622 & 0.716 & 0.663 & 0.658 & 0.528 & 0.676 & 0.593\\
    Greens & 0.379 & 0.346 & 0.510 & 0.447 & 0.523 & 0.318 & 0.319 & 0.340 & 0.517 & \textbf{0.597}\\
    MGM\_Studios & \textbf{0.776} & 0.458 & 0.515 & 0.552 & 0.583 & 0.297 & 0.189 & 0.578 & 0.462 & 0.522\\
    BBCNews & \textbf{0.748} & 0.291 & 0.577 & 0.252 & 0.559 & 0.303 & 0.160 & 0.285 & 0.510 & 0.605\\
    \textbf{Average} & \textbf{0.681} & 0.348 & 0.466 & 0.396 & 0.467 & 0.347 & 0.286 & 0.402 & 0.482 & 0.490\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k5}%
\end{table*}%

==> f1k7.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=7}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 7 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0.393 & 0.182 & 0.424 & 0.086 & 0.363 & 0.236 & 0.162 & 0.179 & 0.391 & \textbf{0.800}\\
    NBA   & 0.788 & 0.410 & 0.786 & 0.769 & \textbf{0.791} & 0.403 & 0.374 & 0.575 & 0.428 & 0.324\\
    TwitterAU & \textbf{0.858} & 0.463 & 0.242 & 0.309 & 0.254 & 0.507 & 0.206 & 0.654 & 0.377 &  0.724\\
    SonyPictures & \textbf{0. 496} & 0.171 & 0.291 & 0.093 & 0.330 & 0.399 & 0.452 & 0.492 & 0.410 & 0.237\\
    AustralianLabor & \textbf{0.897} & 0.442 & 0.503 & 0.452 & 0.614 & 0.386 & 0.466 & 0.404 & 0.601 & 0.677\\
    WhiteHouse & \textbf{0.779} & 0.253 & 0.465 & 0.520 & 0.391 & 0.318 & 0.210 & 0.361 & 0.486 & 0.460\\
    MercedesBenz & \textbf{0.568} & 0.087 & 0.538 & 0.500 & 0.451 & 0.232 & 0.273 & 0.283 & 0.390 & 0.281\\
    Techreview & 0.302 & 0.183 & \textbf{0.410} & 0.320 & 0.380 & 0.211 & 0.174 & 0.216 & 0.314 & 0.209\\
    Cambridge\_Uni & \textbf{0.701} & 0.169 & 0.463 & 0.236 & 0.478 & 0.241 & 0.114 & 0.226 & 0.356 & 0.592\\
    The\_Nationals & \textbf{0.869} & 0.370 & 0.656 & 0.636 & 0.642 & 0.618 & 0.651 & 0.623 & 0.679 & 0.593 \\
    Greens & 0.440 & 0.240 & 0.415 & 0.488 & 0.458 & 0.230 & 0.226 & 0.241 & 0.407 & \textbf{0.636}\\
    MGM\_Studios & \textbf{0.704} & 0.354 & 0.456 & 0.365 & 0.569 & 0.325 & 0.359 & 0.546 & 0.416 & 0.493\\
    BBCNews & \textbf{0.634} & 0.261 & 0.630 & 0.373 & 0.605 & 0.254 & 0.116 & 0.314 & 0.475 & 0.375\\
    \textbf{Average} & \textbf{0.643} & 0.276 & 0.483 & 0.396 & 0.487 & 0.335 & 0.291 & 0.394 & 0.441 & 0.492\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k7}%
\end{table*}%

==> f1k9.tex <==
\begin{table*}[htbp]
  \centering
  \caption{F1 score with $K$=9}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{K = 9 F1 Score} & Ours  & K-Means & BigClam & AgmFit & Censa & FNMTF & GNMF  & DRCC  & Nips & BLOCK-LDA\\
    \midrule
    ABCNews & 0.366 & 0.192 & 0.257 & 0.226 & 0.272 & 0.174 & 0.231 & 0.159 & 0.319 & \textbf{0.729}\\
    NBA   & \textbf{0.941} & 0.437 & 0.709 & 0.652 & 0.689 & 0.419 & 0.399 & 0.501 & 0.432 & 0.493\\
    TwitterAU & \textbf{0.625} & 0.434 & 0.455 & 0.350 & 0.453 & 0.415 & 0.285 & 0.529 & 0.329 & 0.540\\
    SonyPictures & 0.451 & 0.172 & 0.240 & 0.116 & 0.224 & 0.308 & 0.441 & 0.414 & 0.426 & \textbf{0.513}\\
    AustralianLabor & \textbf{0.798} & 0.405 & 0.433 & 0.378 & 0.490 & 0.325 & 0.462 & 0.445 & 0.574 & 0.689\\
    WhiteHouse & \textbf{0.825} & 0.122 & 0.357 & 0.356 & 0.320 & 0.297 & 0.207 & 0.321 & 0.494 & 0.665\\
    MercedesBenz & \textbf{0.714} & 0.115 & 0.521 & 0.410 & 0.430 & 0.249 & 0.263 & 0.375 & 0.396 & 0.359\\
    Techreview & 0.384 & 0.161 & 0.348 & 0.321 & 0.303 & 0.261 & 0.193 & 0.253 & 0.371 & \textbf{0.418}\\
    Cambridge\_Uni & \textbf{0.810} & 0.187 & 0.684 & 0.261 & 0.741 & 0.205 & 0.097 & 0.274 & 0.315 & 0.469\\
    The\_Nationals & 0.549 & 0.385 & 0.586 & 0.468 & 0.404 & 0.624 & 0.566 & 0.578 & \textbf{0.734} & 0.593\\
    Greens & 0.375 & 0.165 & 0.295 & 0.379 & 0.414 & 0.256 & 0.177 & 0.211 & 0.351 & \textbf{0.669}\\
    MGM\_Studios & \textbf{0.723} & 0.275 & 0.239 & 0.258 & 0.534 & 0.270 & 0.473 & 0.671 & 0.389 & 0.478\\
    BBCNews & 0.678 & 0.244 & \textbf{0.760} & 0.459 & 0.732 & 0.237 & 0.093 & 0.279 & 0.406 & 0.426\\
    \textbf{Average} & \textbf{0.634} & 0.254 & 0.453 & 0.402 & 0.462 & 0.311 & 0.299 & 0.385 & 0.426 & 0.542\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1k9}%
\end{table*}%

==> macro_f1_Avs.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Macro F1 Avs}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & LDA & TADW  & RTM \\
    \midrule
    10\% & 0.76084 & 0.75957 & \textbf{0.764392} & 0.369541 & 0.764391 & 0 & 0 & 0 & 0 \\
    20\%   & \textbf{0.810043} & 0.807608 & 0.781474 & 0.366090 & 0.798168 & 0 & 0 & 0 & 0 \\
    30\% & \textbf{0.851001} & 0.837247 & 0.782137 & 0.363368 & 0.809289 & 0 & 0 & 0 & 0 \\
    40\% & \textbf{0.866406} & 0.863792 & 0.785615 & 0.362034 & 0.810925 & 0 & 0 & 0 & 0 \\
    50\% & \textbf{0.877181} & 0.868892 & 0.788058 & 0.363419 & 0.820524 & 0 & 0 & 0 & 0 \\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%

==> macro_f1_M10.tex <==
%\newcolumntype{c}{>{\columncolor{LightCyan}}r}
\begin{table*}[htbp]
  \centering
  \caption{Macro F1 M10}
    \begin{tabular}{lcrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & TADW\\
    \midrule
  %  \rowcolor{LightCyan}
    10\% & \textbf{0.779} & 0.75957 & 0.684668 & 0.333647 & 0.689372 & 0.53234 & 0.7298\\
    20\% & \textbf{0.830} & 0.807608 & 0.729520 & 0.368398 & 0.736581 & 0.561233 & 0.7480 \\
    30\% & \textbf{0.851001} & 0.837247 & 0.756816 & 0.374327 & 0.770119 & 0.568377 & 0.7536 \\
    40\% & \textbf{0.866406} & 0.863792 & 0.768484 & 0.377251 & 0.788898 & 0.575826 & 0.7545 \\
    50\% & \textbf{0.877181} & 0.868892 & 0.762745 & 0.377689 & 0.786972 & 0.582193 & 0.7543\\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%

==> micro_f1_Avs.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Micro F1 Avs}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & LDA & TADW  & RTM \\
    \midrule
    10\% & \textbf{0.791896} & 0.791034 & 0.788818 & 0.498516 & 0.791785 & 0 & 0 & 0 & 0 \\
    20\%   & \textbf{0.841052} & 0.836081 & 0.804554 & 0.498464 & 0.822449 & 0 & 0 & 0 & 0 \\
    30\% & \textbf{0.870722} & 0.861577 &  0.805861 & 0.500305 & 0.833639 & 0 & 0 & 0 & 0 \\
    40\% & \textbf{0.885548} & 0.87989 & 0.808137 & 0.497418 & 0.833957 & 0 & 0 & 0 & 0 \\
    50\% & \textbf{0.892726} & 0.885936 & 0.809081 & 0.500214 & 0.840919 & 0 & 0 & 0 & 0 \\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%

==> micro_f1_M10.tex <==
\begin{table*}[htbp]
  \centering
  \caption{Micro F1 M10}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    Training size & URHN  & TriDNR & Doc2Vec(DV) & DeepWalk(DW) & DV+DW  & LINE & TADW \\
    \midrule
    10\% & \textbf{0.806660} & 0.791034 & 0.717642 & 0.418472 & 0.710098 & 0.604661 & 0.7309 \\
    20\%   & \textbf{0.848206} & 0.836081 & 0.763337 & 0.467022 & 0.761882 & 0.628977 & 0.7482 \\
    30\% & \textbf{0.870722} & 0.861577 &  0.786199 & 0.476375 & 0.795067 & 0.641788 & 0.7490 \\
    40\% & \textbf{0.885548} & 0.87989 & 0.795668 & 0.483834 & 0.812803 & 0.651029 & 0.7591 \\
    50\% & \textbf{0.892726} & 0.885936 & 0.789331 & 0.485936 & 0.810475 & 0.655983 & 0.7606 \\
    \bottomrule
    \end{tabular}%
  \label{tab:f1ground}%
\end{table*}%
